Generate-then-Verify: Reconstructing Data from Limited Published Statistics

We study the problem of reconstructing tabular data from aggregate statistics, in which the attacker aims to identify interesting claims about the sensitive data that can be verified with 100% certainty given the aggregates. Successful attempts in prior work have conducted studies in settings where the set of published statistics is rich enough that entire datasets can be reconstructed with certainty. In our work, we instead focus on the regime where many possible datasets match the published statistics, making it impossible to reconstruct the entire private dataset perfectly (i.e., when approaches in prior work fail). We propose the problem of partial data reconstruction, in which the goal of the adversary is to instead output a $\textit{subset}$ of rows and/or columns that are $\textit{guaranteed to be correct}$. We introduce a novel integer programming approach that first $\textbf{generates}$ a set of claims and then $\textbf{verifies}$ whether each claim holds for all possible datasets consistent with the published aggregates. We evaluate our approach on the housing-level microdata from the U.S. Decennial Census release, demonstrating that privacy violations can still persist even when information published about such data is relatively sparse.

==> docs/experiments.tex <==
\section{Experimental Setup}

\subsection{Dataset and Statistics}

\paragraph{Dataset.} The U.S. Census Bureau has released privacy-protected microdata (Privacy-Protected Microdata File or PPMF) as part of the development of the Disclosure Avoidance System (DAS) for the 2020 Decennial Census. In our experiments, we use the 2023-04-03 version of the 2010 Privacy-Protected Microdata File, which is generated with the differentially private TopDown Algorithm by the Census Bureau and is statistically similar to the private 2010 Decennial Census microdata but. As the private 2010 Census microdata are not public, we treat the Privacy-Protected Microdata as the ground truth during evaluation. 

The PPMF (and Summary File 1, from which the PPMF is derived from) contains data for all people and every housing unit in the United States. Our experiments use the latter, in which each row of the microdata represents one synthetic household response from the 2010 Decennial Census. With the goal of reconstructing data the block level, we select a block from each state, the District of Columbia, and Puerto Rico. Specifically, we take the block that is closest in size to the median block size for each state, District Columbia, and Puerto Rico.

Lastly, the statistics captured in the block-level tables (listed below) are tabulated over the following 10 columns:
%
\input{docs/lists/columns}

\paragraph{Statistics.} In addition to the Privacy-Protected Microdata File, the U.S. Census Bureau releases aggregate statistics of features listed above, calculated from their private microdata, in the form of data tables. These tables are converted into the statistical queries that are used in our integer programming optimization problems. We utilize the following tables:
%
\input{docs/lists/tables}

Each of these tables are released for every block. Each table includes counts for the number of people corresponding to certain feature values defined by the table. For example, cell 2 of table H14 contains the count of owner-occupied family households with a married couple with a householder aged 35-64.


\subsection{IP Solver}

We use Gurobi Optimizer to solve our integer programming optimization problems. We specify parameters ``feasibility tolerance'' and ``integer feasibility tolerance'' 
to their smallest value of $10^{-9}$ to enforce constraints as tightly as possible, and ``pool search mode'' to 2 to find as many best solutions as defined by 
``pool solutions'', which is set to 100 when generating candidates, and to 1 when validating candidates. We also set the time limit parameter as some computations may take too long, particularly for larger blocks. 

\subsection{Baselines}

While we contend that any candidate record that can be reconstructed $100\%$ confidence is already interesting, we would like to further provide context for our results by providing some baseline measure for how likely a block contains any reconstructed record. Let us assume that records in a block are drawn from some prior distribution $P$. Then the multiplicity $m$ of some candidate record $x$ appearing in a block $D$ of size $N$ follows the binomial distribution,
%
\begin{align}\label{eq:binomial}
    P(\multi(x, D)=m) = {N \choose m}p^m(1-p)^{N-m},
\end{align}
%
where $p=P(x)$ is the probability of a single record $x$ being drawn from the prior $P$.

In typical settings in which an adversary has no prior information about the block of interest, $P$ is simply the uniform distribution (i.e., $P(x) = \prod_{j=1}^k |\bfx^{(j)}|$, where $\bfx$ is the one-hot encoded representation of $x$ with columns $\{c_j\}_{j=1}^k$). However, we this baseline to be uninteresting as $P(\multi(x, D)=m)$ is close to $0$ in most cases. In our evaluation, we instead construct a setting in which the prior distribution of the \textit{tract} and \textit{state} that some block $D$ belongs to is known. Let $D_{\text{tract}}$ and $D_{\text{state}}$ be the set of records in the tract and state. Then we can express $p$ as 
%

\begin{align*}
    P(x) = \frac{\multi(x, \tilde{D})}{|\tilde{D}|}
\end{align*}
%
for $\tilde{D} = D_{\text{tract}}$ and $\tilde{D} = D_{\text{state}}$, respectively, and then use Equation \ref{eq:binomial} to calculate the baseline probability for any given candidate $x$.

\tl{TODO: describe holdout split experiments/baselines}

% The second baseline involves splitting a given block into two sets: one private set on which we conduct the reconstruction attack, and one holdout set. After conducting the reconstruction attack and finding candidates that must exist in the private set, we check if the candidate exists at the given multiplicity in the holdout set.

==> docs/intro.tex <==
\section{Introduction}






==> docs/ip.tex <==
\section{Reconstruction via Integer Programming}\label{sec:ip_implementation}

In this section, we describe the implementation of our integer programming methods---namely, solving Problems \ref{eq:ip_problem} and \ref{eq:ip_check_partial_record}. 

\subsection{Setup}\label{sec:ip_setup}

\paragraph{One-hot encoded records.}

As noted previously, while we introduce in Section \ref{sec:prelims} the basic concepts for tabular data reconstruction from aggregate statistics using the histogram representation of records $x \in \cX$, our implementation relies on one-hot encoded representations of $x$. Specifically, let $k$ be the number of columns, which we denote as columns $\{c_j\}_{j=1}^k$, in the domain. Given that all columns in $\cX$ are discrete, we represent records in $\cX$ as one-hot encoded vectors $\bfx = ( \bfx^{(1)} \ldots \bfx^{(k)} )$, where each $\bfx^{(j)}$ encodes the column $c_j$. Thus, we have rows $\bfx \in \{0, 1\}^d$ where $d=\sum_{j=1}^k |\bfx^{(j)}|$ and $k = \sum_{i=1}^d \bfx_i$. Finally, we let the matrix $\bfX \in \{0, 1\}^{N \times d}$ denote a one-hot encoded dataset with $N$ rows.

\paragraph{Query functions.}

In this setting, we consider statistical queries (Definition \ref{def:statistical_queries}) in the form of marginal queries where the predicate function $\phi$ is an indicator function for whether some set of columns takes on some set of values. For example, one can ask the marginal query about the columns \textsc{Sex} and \textsc{Race}: ``How many people are (1) \textsc{Female} and (2) \textsc{White} or \textsc{Black}?" We note that one can break down any predicate $\phi$ into a set of {sub-predicates}, where each sub-predicate corresponds to one unique column pertaining to $\phi$.
Concretely, given some column $c$ and target values $V$, we denote the \textit{sub-predicate} function as
%
\begin{equation*}
    \phi_{c, V}(x) = \bbI\{x_c \in V\},
\end{equation*}
%
where $x_c$ is the value that $x$ takes on for column $c$. Then, any predicate can be rewritten as the product of its sub-predicates (e.g. in the above example, $\phi$ can be written as the product of $\phi_{\textsc{Sex}, \{\textsc{Female}\}}$ and $\phi_{\textsc{Race}, \{\textsc{White, Black}\}}$). 

Given the one-hot encoded representation $\bfx$, $\phi_{c, V}$ can also be rewritten as a
vector $\bfq \in \{0, 1\}^d$ that takes on the value $1$ for indices in $\bfx$ corresponding column $c$ and values $v \in V$ (and $0$ otherwise). In this case, we can then rewrite the sub-predicate function as $\bfx \bfq^T$. \tl{choose different variable C} Likewise, any predicate with $C$ sub-predicates $\bfq_1, \bfq_{2}, \dots, \bfq_C$ can be rewritten as a matrix $\bfQ = \begin{pmatrix} \bfq_1 & \bfq_{2} & \dots & \bfq_c \end{pmatrix}^T \in \{0, 1\}^{C \times d}$. Then $\phi$ can be written as $\bbI \{ \bfx \bfQ^T = \bfone_C \}$ where $\bfone_C$ is a row vector of ones with length $C$. Finally, a statistical query $q_\phi$ can be written as
%
\begin{equation}\label{eq:onehot_query}
    q_\phi(x) = \sum_{j=1}^N \bbI \{ ( \bfX \bfQ^T )_j = \bfone_C \}.
\end{equation}
%
In other words, we check whether each row in $\bfX$ evaluates to $\bfone_C$.\footnote{We note that a simpler alternative to checking $(\bfQ \bfX^T )_j = \bfone_C$ is to check whether the row product is equal to $1$ (i.e. $\prod_k (\bfQ \bfX^T )_{jk} = 1$). However, our integer programming solver (Gurobi) does not support this operation.}

\paragraph{Evaluating multiple queries.} In our setting, the set of queries $Q$ contain queries that can differ in the number of sub-predicates (i.e., columns that are being asked about). For instance, using the above example data domain, one query may ask about the column \textsc{Sex} while another may ask about both \textsc{Sex} and \textsc{Race}. To handle such cases, given some set of queries $Q$, we let $C_\text{max}$ be the maximum number of sub-predicates for queries in $Q$. Then, in cases where some query predicate is comprised of $C < C_\text{max}$ sub-predicates, we can pad its matrix representation $\bfQ$ with rows corresponding to dummy sub-predicates $\bfq_\text{pad} = \bfone_d$. In this way, Equation \ref{eq:onehot_query} still holds (with $\bfone_C$ being replaced by $\bfone_{C_{\text{max}}}$).

Given that now the matrix representation for all queries in $Q$ have the same shape, we can represent $Q$ as a single $3$-dimensional tensor $\bfQ^{(n)} \in \{0, 1\}^{n \times C_{\text{max}} \times d}$. Then, we can calculate the statistics for all queries in $Q$ by evaluating the product $\bfZ = \bfQ^{(n)} \bfX^T \in \{0, 1\}^{n \times C_{\text{max}} \times N}$, where the $i$-th query answer is
%
\begin{equation}\label{eq:onehot_query_set}
    Q(X)_i = \sum_{k=1}^N \bbI \{ \bfZ[i,:,k] = \bfone_{C_{\text{max}}} \}.
\end{equation}
%
Note that we can interpret the vector $\bfZ[i, :, k]$ as a boolean vector that checks whether record $k$ satisfies each of the $C_{\text{max}}$ sub-predicates for query $i$. For ease of notation, we will assume going forward that $C$ refers to $C_{\text{max}}$.

\subsection{Generating Synthetic Data Using Aggregate Statistics (Problem \ref{eq:ip_problem})}

We first describe how we set up the integer programming optimization problem for Problem \ref{eq:ip_problem}---namely, how we represent the constraint $\| Q(D) - Q(D') \|_1 = 0$. Using the notation in Section \ref{sec:ip_setup}, we wish to find some synthetic dataset $X$ (whose one-hot representation we denote as $\bfX$) such that $Q(D) = Q(X)$.

As suggested above, we first evaluate whether each record $\bfX_k$ satisfies all $C$ sub-predicates for each query $q_i$ (i.e., $\bfZ[i,:,k] = \bfone_C$). To do so, we want to add a helper binary variable $\bfW \in \{0, 1\}^{n \times N}$ such that
\begin{equation*}
    \bfW[i, k] = \bbI \{ \bfZ[i,:,k] = \bfone_C \}.
\end{equation*}
%
To enforce this relationship, we add the following constraints,
%
\begin{align}
    \bfW[i, k] \leq& \bfZ[i, j, k], \quad \forall j \in \{ 1, 2, \ldots, C\} \label{eq:query_constraint_1} \\
    \bfW[i, k] \geq& \sum_{j=1}^{C} \bfZ[i, j, k] - (C-1), \label{eq:query_constraint_2}
\end{align}
%
so that $\bfW[i, k]$ evaluates query $q_i$ for record $X_k$. Then, we add the constraints
%
\begin{align}
    Q(D)_i = \sum_{k=1}^{N} \bfW[i,k], \quad \forall i \in \{ 1, 2, \ldots, m\}
\end{align}
%
to ensure that the aggregate count corresponding to query $i$ on the private dataset $D$ match that on $\bfX$.

\paragraph{Explanation if Equations \ref{eq:query_constraint_1} and \ref{eq:query_constraint_2}.} 

Suppose $\bfW[i, k] = 1$. Given that $\bfZ$ is binary, Equation \ref{eq:query_constraint_1} is true if and only if $\bfZ[i, j, k] = 1$ for all $j$, thereby giving us $\bbI \{ \bfZ[i,:,k] = \bfone_C \} = 1$. Moreover, Equation \ref{eq:query_constraint_2} is not violated since we have that
%
\begin{align*}
    1 &\ge \sum_{j=1}^{C} \bfZ[i, j, k] - (C-1) \\
      &\ge C - (C - 1) \quad \text{(} \bfZ \text{ is binary)} \\
      &= 1
\end{align*}
%
Similarly, if $\bfW[i, k] = 0$, then by Equation \ref{eq:query_constraint_2},
\begin{align*}
    0 &\ge \sum_{j=1}^{C} \bfZ[i, j, k] - (C - 1) \\ \implies
    C - 1 &\ge \sum_{j=1}^{C} \bfZ[i, j, k],
\end{align*}
%
which, because $\bfZ$ is binary, can hold if and only if there exists some $j$ such that $\bfZ[i, j, k] = 0$, meaning that $\bbI \{ \bfZ[i,:,k] = \bfone_C \} = 0$. In this case, Equation \ref{eq:query_constraint_1} is not violated since $0 \le \bfZ[i, j, k]$ (again, because $\bfZ$ can only take on the values $0$ and $1$).

\subsubsection{Generating Unique Datasets}

As stated in Section \ref{sec:record_reconstruction}, we set the integer programming solver to output up to $K$ solutions that we then use to generate candidates to verify. However, in the one-hot encoded representation of datasets (as opposed to, for instance, the histogram representation), two datasets with the same set of records that are ordered differently will be considered two unique solutions. To encourage unique solutions, we use a (fixed) vector $\bfh \in \bbN^d$ of randomly generated integers as a hash function, where the hash value for any one-hot encoded record $\bfx$ is $\bfh^T \bfx$. Then, for every $i \in \{1, 2, \ldots, N-1\}$, we add the constraint,
%
\begin{align}
    \bfh^T \bfX_i >= \bfh^T \bfX_{i-1}
\end{align}
%
so that any solution $\cX$ outputted must have its records ordered by their hash values. While this approach is imperfect because, theoretically, different records in $\cX$ may map to the same hash value, we found it to be, in practice, a simple and computationally-efficient approach to filtering out duplicate solutions.

\subsection{Checking the Correctness of Candidate Records (Problem \ref{eq:ip_check_partial_record})}

\tl{TODO: section not completed}

We now switch to setting up constraints for Problem \ref{eq:ip_check_record}---verifying whether some record $\bfx'$ and predicted multiplicity $m$ must exist in the private dataset $D$ according to the released statistics $Q(D)$. In this setting, we have a reconstruction set $R(\bfx', m)$ that is composed of candidate (one-hot encoded) record $\bfx'$ and the predicted multiplicity of that record, $m$. As described in Section \ref{sec:record_reconstruction}, in order to check whether $R(\bfx', m)$ must exist in $D$ according to $Q(D)$, we stipulate in the optimization problem that the number of times $\bfx'$ appears in $\bfX$ cannot equal $m$. If a feasible solution does not exist, then we can conclude that $R(\bfx', m)$ must be correct.

First, we introduce the binary variable $\bfT \in \{0, 1\}^{N \times d}$, where $\bfT_{ij}$ indicates whether $\bfX_{ij} = \bfx'_j$ (i.e., each value of a row in $\cX$ matches the corresponding value in the candidate $\bfx'$). We introduce $\bfU \in \{0, 1\}^{N \times d}$, which is a helper variable used to set $\bfT$ properly in the constraints. In addition, we have a constant $M \gg N$ that will also be needed to set up our constraints properly.

%%%%%%%%%%%%%%%%%%
\tl{Old}


After generating some number of possible datasets, if we see some row appear in all datasets at the same multiplicity, then we take that as a candidate row and multiplicity. Our goal is to verify if the row must exist in the actual dataset at that multiplicity. If there exists a 
generated dataset that does not contain the row at that multiplicity, then we have already generated a possible dataset that could exist without the row at that multiplicity.

A proposed candidate is encoded as a one-hot vector of variable length $L \leq K$, with multiplicity $m$. The length of the candidate encoding varies based on the number of features 
that it contains. In order to check if the candidate must exist in the dataset with multiplicity $m$, we search for a dataset $X'$ that satisfies the counts constraints described above 
and additionally does not contain $m$ rows of the candidate. If no such dataset exists, then we conclude that the candidate must exist in the private dataset $D$ at multiplicity $m$.
 If such a dataset does exist, then we have generated a potential solution without the candidate row at multiplicity $m$ and so it does not necessarily need to exist in $D$ 
 (this generated solution could be $D$ instead). 

We introduce a binary variable $S$ of length $N$, which we use as an indicator for whether or not an entire row of $X'$ matches the candidate row. We additionally introduce 
binary variables $T$ and $U$ of shape $(N, L)$. $T$ indicates if each element of the one-hot encoded candidate row, representing a specific feature value, matches its corresponding feature value index in $X'$. $U$ is a helper binary 
variable for $T$; when an element does not match its corresponding index in $X'$, $U$ manages the possible values that $X'$ can take on.

We first set up constraints with $T$ and $U$ on $X'$. For row $r$ in $X'$, we constrain index $c$, which corresponds to one feature value included in the 
candidate. Let $v$ be the indicator value for the that feature value in the one-hot encoded candidate. Let values $T_{r,i}$ and $U_{r,i}$ correspond to $X'_{r,c}$. Let $M$ be a large constant that enforces
or relaxes constraints. Then we add the following constraints:
\begin{align}
X'_{r,c} - v \leq& M(1-T_{r,i}) \\
v - X'_{r,c} \leq& M(1-T_{r,i}) \\
X'_{r,c} - v \geq&  1 - MT_{r,i} - M(1-T_{r,i})U_{r,i} \\
v - X'_{r,c} \geq& 1 - MT_{r,i} - M(1-T_{r,i})(1-U_{r,i})
\end{align}.

Consider the case when $T_{r,i} = 1$. Then from constraints 5 and 6, we have that $X'_{r,c} \leq v$ and $X'_{r,c} \geq v$, which implies that $X'_{r,c} = v$, which means that the indicator value for the feature value in the one-hot encoding of the candidate is equal to its corresponding value in row $r$ and column $c$ of $X'$. Constraints 7 and 8 give $X'_{r,c} - v \geq 1-M$ and $v - X'_{r,c} \geq 1-M$. 
Given that $M$ is a large constant and that $v$ and $X'_{r,c}$ are both in the domain $\{0, 1\}$, these constraints are essentially not enforced.

When $T_{r,i} = 0$, we have $X'_{r,c} - v \leq M$ and $v - X'_{r,c} \leq M$ from constraints 5 and 6. Since $v$ and $X'_{r,c}$ are both in the domain $\{0, 1\}$, these constraints are 
essentially not enforced. From constraints 7 and 8, we have that $X'_{r,c} - v \geq  1 - MU_{r,i}$ and $v - X'_{r,c} \geq  1 - M(1-U_{r,i})$. Then, for $U_{r,i} = 0$, we have that 
$X'_{r,c} - v \geq  1$ and $v - X'_{r,c} \geq  1 - M$, which implies $1 \leq X'_{r,c} - v \leq M - 1$, enforcing that $X'_{r,c} \neq v$ when $T_{r,i} = 0$. Similarly, for 
$U_{r,i} = 0$, we have $X'_{r,c} - v \geq  1$ and $v - X'_{r,c} \geq 1 - M$ which yields $1 \leq X'_{r,c} - v \leq M - 1$ and enforces $X'_{r,c} \neq v$ when $T_{r,i} = 0$. We 
place these constraints for row in $X'$ and for all indices corresponding to feature values included in the candidate.


First, introduce the binary variable $\bfS \in \{0, 1\}^N$, where $\bfS_i$ indicates whether row $i$ in $\bfX$ equates to the candidate $\bfx'$.

From here, we can place constraints on $S$ based on the values of $T$. If an entire row of $X'$ matches the candidate row, then the entire corresponding row of $T$ should be equal to
1. This can be enforced with the following constraints:
\begin{align}
S_r \leq& T_{r, i} \quad \forall i \in [0, L - 1] \\
S_r \geq& \sum_{i = 0}^{L - 1} T_{r, i} - (L - 1)
\end{align}.

When $S_r = 1$, all values of row $r$ of $T$ must be equal to 1 from constraint 9. When $S_r =0$, we have that at least one of value in row $r$ of $T$ must not be equal to 1 from 
constraint 10.

With $S$ indicating which rows that match the candidate, we check the multiplicity on the candidate row within $X'$ by summing $S$. Two final constraints are needed to ensure the 
solver attempts to find potential datasets that do not include the candidate row at the given multiplicty. Let $Y$ be a scalar binary variable.
\begin{align}
    \sum_{i=0}^{N-1} S_i - m \leq MY - 1 \\
    \sum_{i=0}^{N-1} S_i - m \geq 1 - M(Y - 1)
\end{align}
If $Y=0$, we have $\sum_{i=0}^{N-1} S_i - m  \leq -1$ and $\sum_{i=0}^{N-1} S_i - m  \geq 1 - M$, which gives 
$1 \leq m - \sum_{i=0}^{N-1} S_i \leq m - 1$, enforcing  
$m \neq \sum_{i=0}^{N-1} S_i$. Similarly, if $Y = 1$, we have $\sum_{i=0}^{N-1} S_i - m  \leq M - 1$ and $\sum_{i=0}^{N-1} S_i - m  \geq 1$, which also enforces $m \neq \sum_{i=0}^{N-1} S_i$.

If the solver is unable to find a solution $X'$ under these constraints, then we conclude that there does not exist a dataset without the $m$ rows of the candidate and confirm that 
the candidate must exist at that multiplicity. A similar integer programming problem can be set up to confirm that a candidate at multiplicity $m$ cannot exist by replacing
constraints 11 and 12 with the following single constraint:
\begin{align}
    \sum_{i=0}^{N-1} S_i = m
\end{align}

If the solver cannot find a solution where the candidate row appears exactly $m$ times in the dataset, then we conclude that candidate cannot exist at that multiplicity in the dataset.

==> docs/lists/columns.tex <==

\begin{itemize}[noitemsep, leftmargin=20pt]
  \renewcommand{\labelitemi}{}

\item \textbf{Tenure}: One of 4 tenancy statuses: owned with mortgage, owned free and clear, rented, or occupied without payment of rent

\item \textbf{Vacancy status}: Not vacant, or one of 7 vacancy statuses: for rent, rented but not occupied, for sale, sold and not occupied, for seasonal or occasional use, for migrant workers, or other.

\item \textbf{Household size}: Size of household: 1, 2, 3, 4, 5, 6, or 7 or more

\item \textbf{Household type}: One of 7 types: married couple household, other family household (with a male/female householder), nonfamily household (with a male/female householder, living alone/not living alone).

\item \textbf{Household type (including details about cohabitation and children)}: One of 12 types: married couple (with/without children $<$ 18), cohabiting couple (with/without children $<$ 18), no spouse/partner present (male/female householder, with own children $<$ 18/with relatives and without own children $<18$/only nonrelatives present/living alone)

\item \textbf{Presence of people under 18 years in household}: Whether or not one or more people younger than 18 are in the household

\item \textbf{Presence of people over 65 years in household}: Whether or not one or more people 65 years and over are in the household

\item \textbf{Hispanic householder status}: Whether or not the householder is of Hispanic origin,

\item \textbf{Householder age}: Age of the householder in one of 7 age buckets: 15-24, 24-35, ..., 75-84, or 85 years and older. 

\item \textbf{Householder race}: Race of the householder in one of 7 categories: White alone, Black alone, American Indian or Alaskan Native alone, Asian alone, Native Hawaiian or Pacific Islander alone, some other race alone, or two or more races.

\end{itemize}

==> docs/lists/household_mapping_table.tex <==
\begin{longtable}{lrrrrrrrrrrr}
\toprule
block & n & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
010030102001008 & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 3 & 2 & 2 & 0 \\
 &  & 3 & 5 & 5 & 5 & 5 & 4 & 3 & 2 & 2 & 0 \\
 \hline
020200029004033 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 1 & 0 \\
 &  & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 1 & 0 \\
 \hline
040132168093013 & 13 & 13 & 13 & 12 & 12 & 12 & 12 & 12 & 12 & 0 & 0 \\
 &  & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 \hline
050590203001069 & 6 & 6 & 6 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 \\
 &  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 \\
 \hline
060830020052015 & 19 & 19 & 19 & 16 & 16 & 16 & 15 & 6 & 3 & 0 & 0 \\
 &  & 4 & 13 & 14 & 14 & 14 & 11 & 6 & 3 & 0 & 0 \\
 \hline
080050056304008 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 7 & 7 & 0 & 0 \\
 &  & 4 & 4 & 4 & 4 & 4 & 4 & 1 & 1 & 0 & 0 \\
 \hline
090053061001004 & 17 & 17 & 17 & 17 & 17 & 17 & 1 & 1 & 0 & 0 & 0 \\
 &  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 & 0 \\
 \hline
100050519002096 & 14 & 14 & 14 & 6 & 6 & 6 & 6 & 6 & 2 & 0 & 0 \\
 &  & 0 & 4 & 4 & 4 & 4 & 4 & 4 & 2 & 0 & 0 \\
 \hline
120990077422015 & 14 & 14 & 14 & 14 & 14 & 14 & 14 & 10 & 0 & 0 & 0 \\
 &  & 2 & 2 & 2 & 2 & 2 & 2 & 0 & 0 & 0 & 0 \\
 \hline
131150014002016 & 10 & 10 & 10 & 9 & 9 & 9 & 9 & 4 & 3 & 0 & 0 \\
 &  & 3 & 5 & 4 & 4 & 4 & 3 & 2 & 1 & 0 & 0 \\
 \hline
150090303013006 & 20 & 20 & 20 & 20 & 20 & 20 & 14 & 9 & 5 & 0 & 0 \\
 &  & 2 & 8 & 9 & 9 & 8 & 8 & 4 & 1 & 0 & 0 \\
 \hline
160179505002050 & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 3 & 0 \\
 &  & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 0 & 0 \\
 \hline
170318260003022 & 9 & 9 & 9 & 3 & 3 & 3 & 3 & 2 & 0 & 0 & 0 \\
 &  & 1 & 3 & 3 & 3 & 3 & 3 & 2 & 0 & 0 & 0 \\
 \hline
180190510001046 & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 2 & 2 & 0 & 0 \\
 &  & 5 & 5 & 5 & 5 & 5 & 3 & 2 & 2 & 0 & 0 \\
 \hline
190119606002012 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 0 & 0 \\
 &  & 2 & 2 & 2 & 2 & 2 & 2 & 1 & 1 & 0 & 0 \\
 \hline
200814631002010 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 2 & 0 \\
 &  & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 2 & 0 \\
 \hline
211259710024025 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 4 & 3 & 0 & 0 \\
 &  & 2 & 3 & 3 & 3 & 3 & 3 & 2 & 1 & 0 & 0 \\
 \hline
220530004002010 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 6 & 2 & 0 & 0 \\
 &  & 1 & 4 & 4 & 4 & 4 & 4 & 4 & 0 & 0 & 0 \\
 \hline
230239707002028 & 9 & 9 & 9 & 7 & 7 & 7 & 7 & 7 & 0 & 0 & 0 \\
 &  & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 & 0 \\
 \hline
245102718013027 & 14 & 14 & 14 & 14 & 14 & 14 & 14 & 5 & 3 & 3 & 0 \\
 &  & 4 & 6 & 6 & 6 & 6 & 6 & 3 & 3 & 3 & 0 \\
 \hline
250138125005006 & 16 & 16 & 16 & 16 & 16 & 16 & 12 & 7 & 6 & 0 & 0 \\
 &  & 3 & 3 & 3 & 3 & 2 & 2 & 2 & 1 & 0 & 0 \\
 \hline
261635645021006 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 8 & 4 & 0 \\
 &  & 1 & 6 & 6 & 6 & 6 & 6 & 6 & 3 & 2 & 0 \\
 \hline
270131710003012 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 3 & 0 & 0 & 0 \\
 &  & 2 & 2 & 2 & 2 & 2 & 2 & 1 & 0 & 0 & 0 \\
 \hline
281299503002029 & 7 & 7 & 7 & 3 & 3 & 3 & 0 & 0 & 0 & 0 & 0 \\
 &  & 0 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & 0 \\
 \hline
291754901001087 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 3 & 3 & 0 & 0 \\
 &  & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 \\
 \hline
300310003003154 & 4 & 4 & 4 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 \\
 &  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 \\
 \hline
310539637001302 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 0 \\
 &  & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 0 \\
 \hline
320030058281049 & 15 & 15 & 15 & 15 & 15 & 15 & 15 & 15 & 13 & 2 & 0 \\
 &  & 2 & 9 & 9 & 9 & 9 & 9 & 9 & 6 & 0 & 0 \\
 \hline
330150560002030 & 10 & 10 & 10 & 10 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 \hline
340210025002002 & 17 & 17 & 17 & 17 & 17 & 17 & 10 & 7 & 2 & 1 & 0 \\
 &  & 3 & 6 & 7 & 7 & 7 & 6 & 5 & 2 & 1 & 0 \\
 \hline
350019406001374 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 1 & 1 & 0 \\
 &  & 2 & 3 & 3 & 3 & 3 & 3 & 3 & 1 & 1 & 0 \\
 \hline
360710021001007 & 15 & 15 & 15 & 15 & 15 & 15 & 15 & 15 & 10 & 0 & 0 \\
 &  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 \\
 \hline
370610901004013 & 11 & 11 & 11 & 9 & 9 & 9 & 1 & 0 & 0 & 0 & 0 \\
 &  & 0 & 1 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 \\
 \hline
380539401001087 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 \\
 &  & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2 \\
 \hline
390572009001020 & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 3 & 3 & 0 & 0 \\
 &  & 4 & 4 & 4 & 4 & 4 & 4 & 0 & 0 & 0 & 0 \\
 \hline
400470006004025 & 5 & 5 & 5 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 \\
 &  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 \\
 \hline
410359718001027 & 9 & 9 & 9 & 9 & 9 & 9 & 5 & 4 & 2 & 0 & 0 \\
 &  & 3 & 4 & 4 & 4 & 4 & 3 & 2 & 0 & 0 & 0 \\
 \hline
420770015011076 & 10 & 10 & 10 & 10 & 10 & 10 & 8 & 7 & 5 & 0 & 0 \\
 &  & 3 & 4 & 4 & 4 & 4 & 2 & 2 & 2 & 0 & 0 \\
 \hline
440090515025004 & 16 & 16 & 16 & 16 & 16 & 16 & 16 & 16 & 16 & 0 & 0 \\
 &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 \hline
450339706005045 & 9 & 9 & 9 & 9 & 9 & 9 & 9 & 6 & 1 & 0 & 0 \\
 &  & 7 & 7 & 7 & 7 & 7 & 7 & 6 & 1 & 0 & 0 \\
 \hline
460459621001149 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 0 \\
 &  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 \\
 \hline
470499651003033 & 9 & 9 & 9 & 9 & 9 & 9 & 9 & 9 & 0 & 0 & 0 \\
 &  & 4 & 4 & 4 & 4 & 4 & 2 & 2 & 0 & 0 & 0 \\
 \hline
484391114043013 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 4 & 3 & 0 & 0 \\
 &  & 3 & 3 & 3 & 3 & 3 & 2 & 2 & 1 & 0 & 0 \\
 \hline
490299701001360 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 0 & 0 & 0 & 0 \\
 &  & 2 & 2 & 2 & 2 & 2 & 2 & 0 & 0 & 0 & 0 \\
 \hline
500279665003079 & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 7 & 2 & 0 \\
 &  & 3 & 3 & 3 & 3 & 3 & 3 & 3 & 1 & 0 & 0 \\
 \hline
517600416002006 & 9 & 9 & 9 & 9 & 9 & 9 & 8 & 8 & 4 & 0 & 0 \\
 &  & 7 & 7 & 7 & 7 & 7 & 6 & 6 & 4 & 0 & 0 \\
 \hline
530670104001015 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 1 & 0 \\
 &  & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 1 & 1 & 0 \\
 \hline
540379723001015 & 6 & 6 & 6 & 4 & 4 & 4 & 4 & 4 & 4 & 0 & 0 \\
 &  & 0 & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 0 & 0 \\
 \hline
550170110001013 & 9 & 9 & 9 & 9 & 9 & 9 & 9 & 6 & 0 & 0 & 0 \\
 &  & 6 & 7 & 7 & 7 & 7 & 5 & 1 & 0 & 0 & 0 \\
 \hline
560210013004053 & 5 & 5 & 5 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 \\
 &  & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 \\
\bottomrule
\end{longtable}

\begin{tabular}{rrrrrrrrrrr}
\toprule
Sum: n & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
486 & 486 & 486 & 441 & 431 & 431 & 379 & 274 & 179 & 30 & 2 \\
 & 112 & 167 & 168 & 168 & 166 & 148 & 109 & 61 & 19 & 2 \\
\bottomrule
\end{tabular}

\begin{tabular}{rrrrrrrrrrr}
\toprule
Mean: n & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
9.72 & 9.72 & 9.72 & 8.82 & 8.62 & 8.62 & 7.58 & 5.48 & 3.58 & 0.60 & 0.04 \\
     & 2.24 & 3.34 & 3.36 & 3.36 & 3.32 & 2.96 & 2.18 & 1.22 & 0.38 & 0.04 \\
\bottomrule
\end{tabular}

\begin{tabular}{rrrrrrrrrrrr}
\toprule
Sum: n & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
500 & 500 & 500 & 446 & 425 & 424 & 382 & 284 & 139 & 41 & 12 \\
    & 100 & 167 & 166 & 163 & 161 & 142 & 98 & 42 & 12 & 2 \\
\bottomrule
\end{tabular}

\begin{tabular}{rrrrrrrrrrrr}
\toprule
Mean: n & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule
10.00 & 10.00 & 10.00 & 8.92 & 8.50 & 8.48 & 7.64 & 5.68 & 2.78 & 0.82 & 0.24 \\
      & 2.00 & 3.34 & 3.32 & 3.26 & 3.22 & 2.84 & 1.96 & 0.84 & 0.24 & 0.04 \\
\bottomrule
\end{tabular}

==> docs/lists/tables.tex <==
\begin{itemize}[noitemsep, leftmargin=20pt]
  \renewcommand{\labelitemi}{}

\item \textbf{P16}: Household type,

\item \textbf{P16 A-G}: Household type (iterated by race),

\item \textbf{P16 H}: Household type for households with a householder who is Hispanic or Latino,

\item \textbf{P16 I-O}: Household type for households with a householder who is not Hispanic or Latino (iterated by race),

\item \textbf{P16 P-V}: Household type for households with a householder who is Hispanic or Latino (iterated by race),

\item \textbf{P19}: Households by presence of people 65 years and over, household size, and household type,

\item \textbf{P20}: Households by type and presence of own children under 18 years,

\item \textbf{P21}: Households by presence of people under 18 years,

\item \textbf{H1}: Housing units (total count),

\item \textbf{H3}: Occupancy status,

\item \textbf{H4}: Tenure,

\item \textbf{H4 A-G}: Tenure (iterated by race),

\item \textbf{H4 H}: Tenure of housing units with a householder who is Hispanic or Latino,

\item \textbf{H4 I-O}: Tenure of housing units with a householder who is not Hispanic or Latino (iterated by race),

\item \textbf{H4 P-V}: Tenure of housing units with a householder who is Hispanic or Latino (iterated by race),

\item \textbf{H5}: Vacancy status of vacant housing units,

\item \textbf{H6}: Race of householder,

\item \textbf{H7}: Hispanic or Latino origin of householder by race of householder,

\item \textbf{H9}: Household size,

\item \textbf{H10}: Tenure by race of householder,

\item \textbf{H11}: Tenure by Hispanic or Latino origin of Householder,

\item \textbf{H12}: Tenure by household size,

\item \textbf{H12 A-G}: Tenure by household size (iterated by race),

\item \textbf{H12 H}: Tenure by household size of households with a householder who is Hispanic or Latino,

\item \textbf{H12 I}: Tenure by household size of households with a householder who is White only and not Hispanic or Latino,

\item \textbf{H13}: Tenure by age of householder,

\item \textbf{H13 A-G}: Tenure by age of householder (iterated by race),

\item \textbf{H13 H}: Tenure by age of householder for housing units with a householder who is Hispanic or Latino,

\item \textbf{H13 I}: Tenure by age of householder for housing units with a householder who is White alone and not Hispanic or Latino,

\item \textbf{H14}: Tenure by household type by age of householder,

\item \textbf{H15}: Tenure by presence of people under 18 years, excluding householders, spouses, and unmarried partners,

\end{itemize}

==> docs/prelims.tex <==
\section{Preliminaries}\label{sec:prelims}

% \subsection{Tabular Data Reconstruction}

In this setting, we have some \textit{dataset} $D$ that is comprised of a multiset of $N$ records from a discrete domain $\cX$. 
%
We note that equivalently, we can also represent such datasets $D$ as histograms (vectors) $\bfh^D \in \cH_{\cX}$, where $\cH = \{ \bbN \cup \{0\} \}^{|\cX|}$. Each element $\bfh^D_i$ corresponds to number of times some record type appears in $D$. We let $\idx_{\cH_{\cX}}(x) : \cX \rightarrow \bbN$ be the function that maps each $x \in \cX$ to the corresponding index $i$ for $\cH_{\cX}$. We will use this notation for the histogram representation of $\cX$ in this section to help introduce various definition pertaining to data reconstruction and synthetic data generation via integer programming. We note, however, that in our actual implementation of our integer programming methods (Section \ref{sec:ip_implementation}), we will instead represent the data as one-hot encoded vectors

%
Let $Q$ be some set of $n$ queries corresponding to the data domain $\cX$, and let $Q(D) \in \mathbb{R}^n$ a vector of aggregate statistics on dataset $D$ where each element is a statistic corresponding to a query in $Q$. Formally, we define a statistical query as the following:
%
\begin{definition}[Statistical Queries \citep{SQ}]\label{def:statistical_queries}
Given a predicate function $\phi \colon \cX \rightarrow \{0,1\}$, a statistical query (also known as a linear query or counting query) $q_\phi$ is defined as
\begin{equation*}
   q_\phi(D) = \sum_{x\in D} \phi(x) 
\end{equation*}
for any dataset $D$. 
\end{definition}
%
In other words, these queries are functions that count the number of rows in $D$ that satisfy some given property $\phi$.

Given access only to some set of aggregate statistics $Q(D)$, the goal of the adversary in this setting is then to output some set of rows $x' \in \cX$, that (hopefully) contain rows contained in $D$ (i.e. $\bbI \{x' \in D\}$). We call this set the \textit{reconstruction set} $R$.

To construct $R$, one natural approach is to frame reconstruction as a synthetic dataset generation problem and solve it using integer programming. Specifically, this integer programming problem aims to find a possible solution matrix $X \in \{{\bbN \cup \{0\}}\}^ {N \times d}$ that satisfies $Q(D) = Q(X)$. In its simplest form, reconstruction via integer programming can be set up as an optimization problem with a constant objective,
%
\begin{align}\label{eq:ip_problem}
    X = \arg\min_{D'} \ &0 \\
    \text{s.t.} \ &\| Q(D) - Q(D') \|_1 = 0. \notag
\end{align}

\subsection{Dataset-level Reconstruction}\label{sec:record_reconstruction}

We first consider reconstruction attacks at the \textit{dataset}-level, in which the adversary attempts to reconstruct the entirety of $D$ from $Q(D)$. In other words, they must produce a reconstruction set $R$ of exactly size $N$, which we assume in this setting is known publicly. In this case, we can assess the a reconstruction attack by taking the (mean) $\ell_1$-distance between the histogram representations of $D$ and $R$,
%
\begin{equation*}
    \ell_1\text{-error}(D, R) = \frac{\| \bfh^D - \bfh^R \|_1}{N}.
\end{equation*}

\paragraph{Guaranteeing the correctness of $R$.} 

\citet{abowd20232010} propose a method for guaranteeing the correctness of any generated dataset by checking for the uniqueness of the solution $X$. Their proposition can be summarized as the following procedure: (1) find $X$ by solving Problem \ref{eq:ip_problem}, (2) find some $X'$ that satisfies $Q(D) = Q(X)$ while maximizing the distance between $X$ and $X'$, and (3) check whether $X$ and $X'$ are the same. If $X$ and $X'$ are indeed the same, then we can conclude $X$ is a unique solution to Problem \ref{eq:ip_problem}, and thus $X$ and $D$ must exactly match. More formally, step (2) can written down as
%
\begin{align}\label{eq:ip_uniq_dataset}
    X' = \arg\max_{D'} \ &\| \bfh^D - \bfh^X \|_2 \\
    \text{s.t.} \ &\| Q(D) - Q(D') \|_1 = 0, \notag
\end{align}
%
and (3) corresponds to checking that $\| \bfh^X - \bfh^{X'} \|_1 = 0$.

\subsection{Record-level Reconstruction}

In our work, we instead focus on what we denote as \textit{record}-level reconstruction, where the goal is to instead reconstruct from $Q(D)$ some record $x \in D$ and its multiplicity $m$ (i.e., how many times it appears in $D$). We note that using the same language as above for $dataset$-level reconstruction, we can say that the goal of the adversary is again to output some reconstruction set $R$ but with $1 \le |R| \le N$ and all elements in $R$ being the same.

Let denote this form of reconstruction set $R$ as the multiset $R(\hx, \hm)$ that includes some $\hx \in \cX$ with (predicted) multiplicity $\hm$. In addition, we define $\multi(x, D) : \cX \times \cX^N \rightarrow \bbN \cup \{0\}$ to be the function that outputs the multiplicity of some record $x$ in the dataset $D$. We can then check if the predicted multiplicity of $R(\hx, \hm)$ is exactly correct (i.e., $\bbI \{ \multi(\hx, D) = \hm \}$) or again evaluate $\ell_1$-distance, $| \multi(\hx, D) - \hm |$.

% Let $R(x, m)$ be the multiset the records $x \in \cX$ with (predicted) multiplicity $m$, then we can write the true multiplicity of $x$ as $\bfh^D_i$ where $i = \idx_{\cH_{\cX}}(x)$. We can then check if the predicted multiplicity of $R = R(x, m)$ is exactly correct (i.e., $\bbI \{ \bfh^D_i = m\}$) or again evaluate $\ell_1$-distance. $| \bfh^D_i - m |$. Alternatively, let us denote $U(X)$ as the set of all $R(X,m)$ in some multiset of rows $X$. Then we can equivalently say that the predicted multiplicity of $R$ is exactly correct if $R \in U(D)$.

\paragraph{Guaranteeing the correctness of $R$.}

Like in the \textit{dataset}-level reconstruction attack setting, we can also guarantee the correctness of any reconstruction set $R$ for record-level reconstruction using integer programming. At a high level, given some candidate record $\hx$ and a predicted multiplicity $\hm$, we again solve Problem \ref{eq:ip_problem} but now with the added constraint that $\multi(\hx, D) \ne \hm $. If a feasible solution does not exist, then we can conclude that the candidate $\hx$ must exist in $D$ with multiplicity $\hm$. Formally, this optimization problem can be written as
%
\begin{alignat}{2}\label{eq:ip_check_record}
    X' = \arg\min_{D'} &\ 0 \\
    \text{s.t.} \ &\| Q(D) - Q(D') \|_1 &= 0. \notag \\
    &\multi(\hx, D) \ne \hm \notag
\end{alignat}

\paragraph{Partial Reconstruction.}

Suppose we wish to reconstruct only some subset of columns $C$ in $\cX$. Let us denote this data domain as $\cX_C$. Then we can again write our reconstruction sets as $R(\hx, \hm)$ but with $\hx \in \cX_C$. Let us define $\multi_C(\hx, D) : \cX_C \times \cX_C^N \rightarrow \bbN \cup \{0\}$ as a function that outputs the multiplicity for $\hx$ in $D$ after removing columns $c \notin C$. Then we can write our final optimization problem as
%
\begin{alignat}{2}\label{eq:ip_check_partial_record}
    X' = \arg\min_{D'} &\ 0 \\
    \text{s.t.} \ &\| Q(D) - Q(D') \|_1 &= 0. \notag \\
    &\multi_C(\hx, D) \ne \hm \notag
\end{alignat}
%
Note that when $C$ is the set of all columns in $\cX$, we recover Problem \ref{eq:ip_check_record}.


\paragraph{Generating candidate records $R$ to check.} 

Suppose our goal is to find all reconstruction sets $R$ that \textit{must exist} in $D$ according to $Q(D)$. Let us denote $U(D)$ as the set of all $R(x,m)$ for $x \in X$ where $m = \multi(x, D)$ (i.e., the set of all unique records $x \in D$ and their multiplicities). Then the predicted multiplicity of any reconstruction set $R$ is exactly correct if $R \in U(D)$. Using this notation, our goal is equivalent to finding all $R$ such that $\forall D' \in \cX^N$ s.t. $Q(D') = Q(D)$, $R \in U(D')$. In other words, the only way we can be certain that some $R$ is contained in the private dataset $D$ is that it appears in all datasets $D'$ were the statistics $Q(D')$ match $Q(D)$. 

Therefore, to generate candidate records, one can simply generate some synthetic dataset $X$ by solving Problem \ref{eq:ip_problem} and taking all unique records in $\hx \in X$ and their multiplicities $\hm$ (i.e., $U(X)$). Furthermore, to narrow down the set of candidates to check, one can generate many synthetic datasets $X_i$ and take their intersection $\bigcap_{i}^K U(X_i)$ since if there exists some $R \in U(X_i)$ such that $R \notin \bigcap_{i-1}^K U(X_i)$, then $R$ violates the above condition. Later on, we will use this strategy of producing candidates by generating multiple synthetic datasets so that we can manage the computational trade-off between generate the list of candidates and checking them.

==> docs/results.tex <==
\section{Empirical Results}\label{sec:results}

Figure 1 notes:
\begin{itemize}
    \item Figure 1 (left), not sure what
    \item Figure 1 (right). Up to 7 columns, you can reconstruct some record for over (two thirds ish).
    \item Figure 1 (right). For 5 or under, you can reconstruct some record for over 90 percent
    \item Figure 1 (right). For 1-3, you can always find a record
\end{itemize}

Figure 2 notes:
\begin{itemize}
    \item the median is quite low - nearly zero for 6 attributes or more
    \item even for 3-5, it's under 10 percent
    \item at best, sometimes it's around 0.4 (outliers), which is still worse than a coin flip
    \item we found no difference between using the tract and state (\tl{we should confirm what the numbers are for 6 cols and up}
\end{itemize}

Figure 3 notes:
\begin{itemize}
    \item Even filtering out for only unique records, the results do not substantially change. with 6 or less columns, we can reconstruct some candidate for two thirds of the blocks. even for 7 or 8, we can get 60 percent and 10 percent respectively
    \item unique candidate are still vulnerable 
\end{itemize}

Figure 4 is same as Figure 2. Maybe highlight that the baseline is not better in this scenario.

Holdout plots, all the result and baselines look the same as Figures 1-4. Box plot where each point is a random seed for a block. It shows that for some blocks, reconstruction is trivial (different word), but for most, it's not. 

\begin{figure}
\begin{center}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/box_num_candidates_filter.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/min_1_candidate_filter.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/box_probabilities_Tract.png}
  \caption{Tract-Level Distribution}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/box_probabilities_State.png}
  \caption{State-Level Distribution}
  \label{fig:sub2}
\end{subfigure}
\caption{
(a) Total number of candidates verified across all blocks by number of reconstructed features.
% Excludes blocks which no candidates of a specific number of reconstructed features are verified.
(b) Number of blocks (out of 50) for which we can reconstruct at least one candidate that contains each number of features. (c) and (d): Distributions of the probabilities of (verified) candidates appearing in a synthetic block (of the same size N) sampled from the (c) tract and (d) block that the block belongs to (binomial distribution).
\\
As shown in (b), we can reconstruct some record for over two-thirds of the 50 blocks for up to 8 columns. For up to 7 columns, we can reconstruct at least one record for over 90 percent of blocks. For up to 3 columns, a record can be reconstructed in every block. \\ We see the overall distributions between sampling from the tract and the state are not different. The median probability across reconstructed candidates of all numbers of columns is very low: under 0.1, except for candidates with one column. For 4 or more attributes, the maximum probability that a candidate appears never above 0.5.
}
\end{center}
\end{figure}




\begin{figure}
\begin{center}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/box_num_unique_candidates_filter.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/min_1_unique_candidate_filter.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/box_unique_probabilities_Tract.png}
  \caption{Tract-Level Distribution}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/box_unique_probabilities_State.png}
  \caption{State-Level Distribution}
  \label{fig:sub2}
\end{subfigure}
\caption{
(a) Total number of unique candidates (multiplicity of one) verified across all blocks by number of reconstructed features.
% Excludes blocks which no candidates of a specific number of reconstructed features are verified.
(b) Number of blocks (out of 50) for which we can reconstruct at least one candidate that contains each number of features. (c) and (d): Distributions of the probabilities of (verified) candidates appearing in a synthetic block (of the same size N) sampled from the (c) tract and (d) block that the block belongs to (binomial distribution).
\\
In (b), we see that for up to 7 columns, we can reconstruct at least one unique candidate for over 80 percent of the blocks. For 8 and 9 columns, we can reconstruct 60 percent and 10 percent respectively. This demonstrates that unique candidates are still vulnerable to reconstruction. \\ (c) and (d) shows that even for unique records, the baseline of sampling a random dataset from a larger distribution does not perform better. We see similar distributions as in Figure 2, with low medians across candidates of all numbers of attributes as well.
}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/box_num_candidates_split.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/min_1_candidate_split.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/box_in_holdout.png}
    \caption{}
\end{subfigure}
\caption{
(a) Total number of candidates verified across all 10 splits of all 50 blocks, by number of reconstructed features. Each split contains half of one block, where the other half of the block is treated as a holdout set.
% Excludes blocks which no candidates of a specific number of reconstructed features are verified.
(b) Number of splits (out of 500, 10 for each block) for which we can reconstruct at least one candidate that contains a given number of features.
\\
(c) Distribution of appearance rate of unique candidates in holdout sets averaged across seeds for all blocks per number of features reconstructed. For each block, we have 10 random splits, defined by a random seed, that form private and holdout sets. We attack each of the 10 private sets, generating and verifying candidates. For each candidate, we check if it is in the corresponding holdout set. We take all verified candidates in the 10 splits, group them by number of reconstructed features, and calculate the proportion of this set of candidates that appear in their holdout set for the block. We repeat this for all blocks so that each datum in the plot represents one block.
\\
As shown by the low medians in (c), reconstruction (by this metric) is still nontrivial for most blocks. However, from the outliers, especially for when evaluating candidates with higher numbers of features, reconstructing certain candidates can be easy without usage of any algorithm (for example, there is one block where 10 out of 11 of the original candidates (before splitting) are exactly same, making the holdout split baseline for this block very strong).
}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/box_num_unique_candidates_split.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/min_1_unique_candidate_split.png}
  \caption{}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/box_in_holdout_unique.png}
    \caption{}
\end{subfigure}
\caption{
(a) Total number of unique candidates verified across all 10 splits of all 50 blocks, by number of reconstructed features. Each split contains half of one block, where the other half of the block is treated as a holdout set.
% Excludes blocks which no candidates of a specific number of reconstructed features are verified.
(b) Number of splits (out of 500, 10 for each block) for which we can reconstruct at least one candidate that contains a given number of features.
\\
(c) Distribution of appearance rate of unique candidates in holdout sets averaged across seeds for all blocks per number of features reconstructed. For each block, we have 10 random splits, defined by a random seed, that form private and holdout sets. We attack each of the 10 private sets, generating and verifying candidates. For each candidate, we check if it is in the corresponding holdout set. We take all verified candidates in the 10 splits, group them by number of reconstructed features, and calculate the proportion of this set of candidates that appear in their holdout set for the block. We repeat this for all blocks so that each datum in the plot represents one block.
\\
As shown by the low medians in (c), reconstruction (by this metric) is still nontrivial for most blocks. However, from the outliers, especially for when evaluating candidates with higher numbers of features, reconstructing certain candidates can be easy without usage of any algorithm (for example, there is one block where 10 out of 11 of the original candidates (before splitting) are exactly same, making the holdout split baseline for this block very strong).
}
\end{center}
\end{figure}

\input{docs/example_results}
\subsection{Main Results (todo: rename)}

\subsection{Splitting  (todo: rename)}


% \section{Difficulty of the Problem} 
% % TODO add comparison to person level/census paper

% A first attempt at reconstruction might be to reconstruct candidates that include all 9 attributes in each block by simply generating a single synthetic dataset via integer programming and examining the labels (in private dataset $D$ or not). With this method, we find the multiplicities of most candidates generated are not correct; across the median-sized block at the household level for all 50 states, Puerto Rico, and Washington D.C., 32 out of 481 candidates (7.1\%) were correct and actually in $D$. In 28 of 51 blocks, no candidates were correct.

% \subsection{General}
% We generated and checked candidates for the median-sized block at the household level for all 50 states and Puerto Rico. Note that Washington D.C.'s median-sized block was comparably large, so a slightly modified process was conducted for its experiment. All combinations of up to all 9 features were considered for these states. As shown in Figure 1, we were able to reconstruct and validate at least one candidate that contained up to 3 features in all blocks and up to 7 blocks in a majority (34 of 51) of blocks. We see a large decrease in the number of candidates that could be validated at 8 and 9 features. Figure 2 shows that we also we can reconstruct a unique candidate (a candidate that has a multiplicity of 1 within that block) with up to 7 features for a majority of blocks.

% \begin{figure}
% \begin{center}
% \includegraphics[scale=0.8]{plts/min_1_candidate.png}
%     \caption{Number of blocks (out of 51) for which we can reconstruct at least one candidate that contains a given number of features. }
% \end{center}
% \end{figure}

% \begin{figure}
% \begin{center}
% \includegraphics[scale=0.8]{plts/min_1_unique_candidate.png}
%     \caption{Number of blocks (out of 51) for which we can reconstruct at least one unique candidate that contains a given number of features. }
% \end{center}
% \end{figure}

% The median-sized block for Washington D.C., which included 35 households, was comparably large and required more time on average to validate a candidate. As a result, only candidates that included at least 5 features were checked for correctness, with a timeout of 30 minutes. Similar to most other blocks, we were able to validate at least one candidate with 5, 6, and 7 features.

% \subsection{Example Reconstructed Households}
% The validated households are often unique or have a low multiplicity (1-3) within a block, which allow for specific and interesting insights when combined with column values. Potentially sensitive data in the features includes presence of children, the householder's sex, age, marital status, whether they are living alone, and whether they are Hispanic or not. For example, for the median-sized block in North Dakota, we were able to reconstruct two households with all 9 attributes. Specifically, we found these households were renting, not vacant, had 4 people in the household, were an unmarried, cohabiting couple household with own children under the age of 18, did not have any 65 or older in the household, and the householder was male and not Hispanic. For one of the households, the householder was between 15 and 24 years old, and the other was between 25 and 34 years old. 

% As another example, in South Dakota, we were able to validate a household that owned their residence and paying off a mortgage, with 3 people, was a nonfamily household, with no people under 18 or over 65, and had a male, Hispanic householder between 60 and 64 years old. Also in this block were 2 households with mortgages, 2 people (a married couple), no people under 18 or over 65, with a householder that was not Hispanic and between the ages of 45 and 54. 

\input{docs/lists/household_mapping_table}

==> main/IEEE/figures/atleast1.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{arxiv/figures/images/min_1_candidate_filter.png}
    \caption{
        The number of blocks (out of 50) for which we can verify at least one claim with some number of columns. We can verify at least one claim with up to 8 columns in the majority of the blocks.
    }
    \label{fig:atleast1}
\end{figure}

==> main/IEEE/figures/atleast1_unique.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{arxiv/figures/images/min_1_unique_candidate_filter.png}
    \caption{
        The number of blocks (out of 50) for which we can verify at least one singleton claim with some number of columns. We can verify at least one singleton claim with up to 8 columns in the majority of the blocks.
    }
    \label{fig:atleast1_unique}
\end{figure}

==> main/IEEE/figures/block_size.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{arxiv/figures/images/block_size_unique_hist.png}
    \caption{
        TODO
    }
    \label{fig:blocksize_unique}
\end{figure}
